High-dimensional Location Estimation via Norm Concentration for Subgamma Vectors

In location estimation, we are given $n$ samples from a known distribution $f$ shifted by an unknown translation $\lambda$, and want to estimate $\lambda$ as precisely as possible. Asymptotically, the maximum likelihood estimate achieves the Cram\'er-Rao bound of error $\mathcal N(0, \frac{1}{n\mathcal I})$, where $\mathcal I$ is the Fisher information of $f$. However, the $n$ required for convergence depends on $f$, and may be arbitrarily large. We build on the theory using \emph{smoothed} estimators to bound the error for finite $n$ in terms of $\mathcal I_r$, the Fisher information of the $r$-smoothed distribution. As $n \to \infty$, $r \to 0$ at an explicit rate and this converges to the Cram\'er-Rao bound. We (1) improve the prior work for 1-dimensional $f$ to converge for constant failure probability in addition to high probability, and (2) extend the theory to high-dimensional distributions. In the process, we prove a new bound on the norm of a high-dimensional random variable whose 1-dimensional projections are subgamma, which may be of independent interest.

==> libtheorems.tex <==
% Code for theorems in multiple places
% Originally by Eric Price, placed in the public domain
%
% This lets you write the statement of a theorem/lemma in one place
% and insert it in multiple parts of a document.  This lets you
% include the statement of Lemma 3.2 in both the introduction and the
% place that it's proven, and the numbering can refer to the place
% where it's proven.
%
% Usage:
%
%  \define[optional title]{thm:main}{Theorem}{We show \[ x^2 + y^2 \geq 2xy \].}
%     Before you use it.
%
%  \state{thm:main}
%     in the place where you want the label to be generated
%
%  \restate{thm:main}
%     elsewhere.
%
%  To have consistent equation labels, use $\thmlabel{eq:1}$ rather
%  than $\label{eq:1}$.
%
%
%%%%% Begin code
\usepackage{etoolbox}

\makeatletter

% Define the various variables to be used in \state/\restate
\newcommand{\define}[4][ignore]{%
  \ifstrequal{#1}{ignore}{}{
  \@namedef{thmtitle@#2}{#1}}%
  \@namedef{thm@#2}{#4}%
  \@namedef{thmtypen@#2}{lemma}%
  \newtheorem{thmtype@#2}[theorem]{#3}%
  \newtheorem*{thmtypealt@#2}{#3~\ref{#2}}%
}

% State the theorem, generating the proper number.
\newcommand{\state}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
  \begin{thmtype@#1}
    }{
  \begin{thmtype@#1}[\@nameuse{thmtitle@#1}]
  }
    \label{#1}
    \@nameuse{thm@#1}
  \end{thmtype@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% Include the theorem, with the original numbering
\newcommand{\restate}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
    \begin{thmtypealt@#1}
    }{
  \begin{thmtypealt@#1}[\@nameuse{thmtitle@#1}]
  }
    \@nameuse{thm@#1}
  \end{thmtypealt@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% For equations, this generates a new number if this is the first time
% the theorem is included, and reuses the old number otherwise.
\newcommand{\thmlabel}[1]{
  \@ifundefined{thmdone@\@nameuse{curthm}}{\label{#1}
    }{\tag*{\eqref{#1}}}
}
\makeatother
%%%%% End code


==> norm_concentration_contradiction_approach.tex <==
\section{New approach}
\begin{lemma}
    Let $X \in \R^d$ be a random variable such that for every $v \in \R^{d-1}$, and $\lam \ge 0$, $$\E_X[\exp(\lam (v^T X))] \le \exp(\lam^2\|v\|^2/2) $$
    Let $\delta = e^{-o(d)}$. Then, we have that for any $0< \xi < 1$, with probability $1 - \delta$,
    $$\|X\| \le \sqrt{d} \left(1 + O\left(\frac{1}{\log^{\xi} d} \right) \right)$$
\end{lemma}

\begin{proof}
    Let $\eps, \zeta > 0$, and suppose, for the sake of contradiction, that with probability greater than $\zeta$,
    $$\|X\| > d^{\frac{1}{2} + \eps}$$
    Then, we will pick a random $v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})$, and lower bound the probability that $v^T X > \|v\|\sqrt{2 \log \frac{1}{\delta}}$. %By symmetry, we have that for a random direction $v \sim S^{d-1}$, $v^T X = \|X\| v^T e_1$. So, 
    %\begin{align*}
    %    \Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right] &= \Pr_{X, v \sim S^{d-1}} \left[\|X\| v^T e_1 > \sqrt{ 2 \log \frac{1}{\delta}} \right]\\
    %    &= \Pr_{X, w \sim \mathcal N\left(0,\frac{1}{d}I_{d \times d}\right) }\left[\|X\| \frac{w^T e_1}{\|w\|} > \sqrt{2 \log \frac{1}{\delta}}\right]
    %\end{align*}
    %Now, since $w \sim \mathcal N\left(0, \frac{1}{d}I_{d \times d} \right)$, we have that $\|w\|^2 \sim \chi^2_d/d$. So, with probability at least $1/2$, %$1 - e^{-\Omega(d \eps^2)}$, $$\|w\| \le 1 + \eps$$
    %$$\|w\| \le 1 + O\left(\frac{1}{\sqrt{d}}\right)$$
    %so that
    %$$\|w\| \ge 1 -  \Omega\left(\sqrt{\frac{1}{d} \log \frac{1}{\beta}}\right)$$
    %So, using this and our assumption,
    \begin{align*}
        \Pr_{X, v} \left[v^T X > \|v\| \sqrt{2 \log \frac{1}{\delta}} \right] &\ge \Pr_{X, v} \left[v^T X > \|v\| \sqrt{2 \log \frac{1}{\delta}} \Big | \|X\| > d^{\frac{1}{2} + \eps}  \right] \Pr\left[\|X\| > d^{\frac{1}{2} + \eps} \right]\\
        &> \zeta \Pr_{X, v} \left[v^T X > \|v\| \sqrt{2 \log \frac{1}{\delta}} \Big | \|X\| > d^{\frac{1}{2} + \eps}  \right]
    \end{align*}
    By symmetry, for a random $v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})$, $v^T X = \|X\| v^T e_1$. So,
    \begin{align*}
    \Pr_{X, v} \left[v^T X > \|v\|\sqrt{2 \log \frac{1}{\delta}} \Big | \|X\| > d^{\frac{1}{2} + \eps} \right] &= \Pr_{X, v} \left[\|X\| v^T e_1 > \|v\|\sqrt{2 \log \frac{1}{\delta}} \Big | \|X\| > d^{\frac{1}{2} + \eps}\right]\\
    &= 1 - \Pr_{X, v} \left[\|X\| v^T e_1 \le \|v\|\sqrt{2 \log \frac{1}{\delta}} \Big| \|X\| > d^{\frac{1}{2} + \eps} \right]
    \end{align*}
    Now, let $0 < \xi < 1$, and we will set $\eps = \frac{1}{\log^{1+\xi} d}$. We have
    \begin{align*}
        &\Pr_{X, v} \left[\|X\| v^T e_1 \le \|v\| \sqrt{2 \log \frac{1}{\delta}} \Big| \|X\| > d^{\frac{1}{2} + \eps}\right] \\
        &\le \Pr_{v}\left[d^{\frac{1}{2} + \eps} v^T e_1 \le \|v\| \sqrt{2 \log \frac{1}{\delta}} \right]\\
        &\le \Pr_{v} \left[d^{\frac{1}{2} + \eps} v^T e_1 \le \|v\| \sqrt{2\log \frac{1}{\delta}} \text{ and } \|v\| \le d^{\eps} \sqrt{1 - \eps\log^{1-\xi} d} \right] + \Pr_{v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}\left[\|v\| > d^{\eps} \sqrt{1 - \eps \log^{1-\xi} d}  \right]\\
        &\le \Pr_{v}\left[d^{\frac{1}{2} + \eps}v^T e_1 \le d^{\eps} \sqrt{1 - \eps \log^{1-\xi} d}\sqrt{2 \log \frac{1}{\delta}} \text{ and } \|v\| \le d^{\eps} \sqrt{1 - \eps \log^{1-\xi} d} \right] + \Pr_v\left[\|v\| > 1 + \Omega(\eps \log d)\right]\\
        &\quad  \text{since } d^\eps \ge 1 + \eps \log d \text{ and } \log^{1 - \xi} d \ll \log d\\
        %&\le \Pr_{v}\left[d^{\frac{1}{2} + \eps}v^T e_1 \le d^{\eps} \sqrt{1 - \eps \sqrt{\log d}}\sqrt{2 \log \frac{1}{\delta}} \text{ and } \|v\| \le d^{\eps} \sqrt{1 - \eps \sqrt{\log d}} \right] + e^{-\Omega(\eps^2 d \log^2 d)}\\
        &\le \Pr_{y \sim \mathcal N(0, 1)}\left[y \le  \sqrt{2\left(1 - \eps \log^{1-\xi} d\right)\log \frac{1}{\delta}} \right] + e^{-\Omega(\eps^2 d \log^2 d)} \quad \text{since } \eps \log d = \log^{-\xi} d \ll 1\\
        %&\le \Pr_{y \sim \mathcal N\left(0, \left(\gamma \log \frac{1}{\delta}\right)^{2\eps}\right)}\left[y \le \left(\gamma \log \frac{1}{\delta} \right)^{2\eps} \sqrt{2 \log \frac{1}{\delta}} \right] + blah \quad \text{since } d \ge \gamma \log \frac{1}{\delta}\\
        &\le  (1 - \Omega(\delta^{1-\eps \log^{1-\xi} d})) + e^{-\Omega(\eps^2 d \log^2 d)}
        %&\le \Pr_{X, w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})} \left[\|X\| \frac{w^T e_1}{\|w\|} \le \sqrt{2 \log \frac{1}{\delta}} \Big| \|X\| > \sqrt{d} + \sqrt{2 \log \frac{1}{\delta}}, \|w\| \le 1 + \eps \right] + \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{ d \times d})}\left[\|w\| > 1 + \eps \right]\\
        %&\le \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) w^T e_1 \le (1 + \eps) \sqrt{2 \log \frac{1}{\delta}} \Big | \|w\| \le 1+\eps \right] + e^{-\Omega(d \eps^2)}\\
        %&\le e^{\Omega(d \eps^2)} \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) w^T e_1 \le (1 + \eps) \sqrt{2 \log \frac{1}{\delta}} \right] + e^{-\Omega(d \eps^2)}
    \end{align*}
    So, for our setting of $\eps = \frac{1}{ \log^{1+\xi} d}$, we have shown
    \begin{align*}
        \Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right] > \zeta\left(\Omega\left(\delta^{1 -  \frac{1}{ \log^{2\xi} d}}\right) - e^{-\Omega\left(d/\log^{2 \xi} d \right)}\right)
    \end{align*}
    Here, the first term dominates when $\delta \gg e^{-d/\log^{2 \xi} d}$. Setting $\zeta = \Omega\left(\delta^{\frac{1}{ \log^{2 \xi} d}}\right)$ yields there exists $v_* \in \R^d$ with $$\Pr_X\left[v_*^T X > \|v\|\sqrt{2 \log \frac{1}{\delta}} \right]\ge \Pr_{X, v\sim S^{d-1}} \left[v^T X > \|v\|\sqrt{2 \log \frac{1}{\delta}} \right] > \delta$$
    which contradicts our assumption that for every $\lam \ge 0$,
    $$\E_X \left[\exp(\lam(v_*^T X)) \right]\le \exp(\lam^2\|v\|^2/2)$$
    So, we have shown that for any $0<\xi < 1$, and $\delta \gg e^{-d/\log^{2\xi} d}$, with probability $1 - \Omega(\delta^{\frac{1}{\log^{2\xi} d}})$,
    $$\|X\| \le d^{\frac{1}{2} + \frac{1}{\log^{1+\xi} d}} \le \sqrt{d} \left(1 + O\left(\frac{1}{\log^{\xi} d} \right) \right)$$
    Reparameterizing, we have that for $0 < \xi < 1$ and $\delta' \gg e^{-d}$, with probability $1 - \delta'$,
    $$\|X\| \le \sqrt{d} \left(1 + O\left(\frac{1}{\log^\xi d} \right) \right)$$
    %Now, we can bound the probability above by union bounding over two events: XXX FINISH
    %\begin{itemize}
    %    \item $\|w\| \le 1 + \eps$
    %    \item When $\|w\| > 1 + \eps$
    %\end{itemize}
    %\begin{align*}
    %    &>  \gamma\left(\frac{1}{2} +  \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})} \left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) \frac{w^T e_1}{1+O(1/\sqrt{d})} > \sqrt{2 \log \frac{1}{\delta}}  \right]\right)\\
    %    &\ge \frac{\gamma}{2} \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}}  \right) u> \sqrt{2 \log \frac{1}{\delta}}\left(1+O\left(1/\sqrt{d}\right)\right) \right]\\
    %    %&= (\delta + \gamma) (1 - \beta) \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) u > \sqrt{2 \log \frac{1}{\delta}}-  \Omega\left( \sqrt{\frac{1}{d} \log \frac{1}{\delta} \log \frac{1}{\beta}} \right)\right]\\
    %    &\ge \frac{\gamma}{2} \Pr_{y \sim \mathcal N\left(0, 1 + 2 \sqrt{\frac{2\log \frac{1}{\delta}}{d}} +\frac{2 \log \frac{1}{\delta}}{d}\right)}\left[ y > \sqrt{2 \log \frac{1}{\delta}}\left(1+O\left(1/\sqrt{d} \right)\right) \right]\\
    %    &\ge \frac{\gamma}{2} (1 - 2\delta)
    %    %&\ge \gamma(1 - e^{-\Omega(d\eps^2)})(1 - e^{-\Omega(d)})\\
    %    %&\ge \gamma(1 - e^{-\Omega(d\eps^2)})(1 - \delta)\\
    %\end{align*}
    %where the last inequality follows from the fact that with probability $1 - 2 \delta$, $$y \ge \sqrt{2 \log \frac{1}{\delta}} \sqrt{1 + 2 \sqrt{\frac{2 \log \frac{1}{\delta}}{d}} + \frac{2 \log \frac{1}{\delta}}{d}} > \sqrt{2 \log \frac{1}{\delta}}\left(1 + O(1/\sqrt{d}) \right)$$
    %
    %So, since $\delta < 1/2$, setting $\gamma = 8 \delta$ yields that 
    %$$\Pr_{X, v \sim S^{d-1}}\left[ v^T X > \sqrt{2 \log \frac{1}{\delta}}\right] > \delta$$
    %But this means that there exists a $v_* \in S^{d-1}$ such that
    %$$\Pr_X\left[v_*^T X > \sqrt{2 \log \frac{1}{\delta}} \right] >\delta$$
    %which contradicts our assumption that \emph{for all} $v \in S^{d-1}$ and $\lam \ge 0$,
    %$$\E_X\left[\exp(\lam(v^T X)) \right] \le \exp(\lam^2/2)$$
    %So, we have shown that with probability at least $1 - \delta$,
    %$$\|X\| \le \sqrt{d} + \sqrt{2 \log(8/\delta)}$$
\end{proof}

\subsection{Scratch}
Naively applying the argument will give the right result when $$\delta \gg e^{-\frac{d^2}{\|\Sigma\|_F^2}}$$

\begin{lemma}
    Let $\Sigma \in \R^{d\times d}$. We have
     $$\E_{v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}[v^T \Sigma v] = \frac{\tr(\Sigma)}{d}$$
     and with probability $1 - \delta$, for $v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})$
     $$\left|v^T \Sigma v - \frac{\tr(\Sigma)}{d}  \right| \lesssim \frac{\|\Sigma\|_F}{d} \sqrt{\log \frac{1}{\delta}} + \frac{\|\Sigma\|}{d} \log \frac{1}{\delta}$$
\end{lemma}

\begin{proof}
    Let $u_1, \dots, u_d$ be the eigenvectors of $\Sigma$, with corresponding eigenvalues $\lam_1, \dots, \lam_d$. We have
    \begin{align*}
        \E_{v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}\left[v^T \Sigma v \right] &=\sum_{i=1}^d \lam_i \E_{v \sim \mathcal N(0, \frac{1}{d} I_{d \times d})}\left[(v^T u_i)^2 \right] = \sum_{i=1}^d \lam_i \E_{y \sim \mathcal N(0, \frac{1}{d})}[y^2] = \sum_{i=1}^d \frac{\lam_i}{d} = \frac{\tr(\Sigma)}{d}
    \end{align*}
    So, by the Hanson-Wright inequality (Theorem~\ref{thm:hanson-wright}), the claim follows.
    %\begin{align*}
        %\Pr_{v\sim \mathcal N(0, \frac{1}{d} I_{d \times d}}\left[\left|v^T \Sigma v - \frac{\tr(\Sigma)}{d}\right| > t \right] \le 2 \exp\left( \right)
    %\end{align*}
\end{proof}
\begin{lemma}
    Let $X \in \R^d$ be a random variable such that for every $v \in \R^d$, and $\lam \ge 0$, $$\E_X[\exp(\lam (v^T X))] \le \exp\left(\frac{\lam^2}{2} (v^T \Sigma v)\right) $$
    Then, for $\delta = e^{-o(d)}$, we have that with probability $1 - \delta$,
    $$\|X\| \le \sqrt{\tr(\Sigma)} + (1+o(1))\sqrt{2\|\Sigma\|\log(1/\delta)}$$
\end{lemma}

\begin{proof}
        Let $\eps > 0$, $\gamma > e^{-O(d)}$, and suppose, for the sake of contradiction, that with probability greater than $\delta + \gamma$,
    $$\|X\| > \tr(\Sigma)^{\frac{1}{2} +\eps} + \sqrt{2 \log(1/\delta)}$$
    Then, we will pick a random direction $v \in S^{d-1}$, and lower bound the probability that $v^T X > \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta}}$. 
    \begin{align*}
        &\Pr_{X, v \sim S^{d-1}}\left[v^T X > \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta}} \right]\\
        &\ge \Pr_{X, v \sim S^{d-1}}\left[ v^T X > \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta}} \Big | \|X\| > \tr(\Sigma)^{\frac{1}{2} + \eps} + \sqrt{2 \log \frac{1}{\delta}}\right] \Pr_X \left[ \|X\| > \tr(\Sigma)^{\frac{1}{2} + \eps} + \sqrt{2 \log \frac{1}{\delta}}\right]\\
        &> \gamma \Pr_{X, v\sim S^{d-1}} \left[v^T X > \sqrt{(v^T \Sigma v) \cdot 2\log \frac{1}{\delta}} \Big | \|X\| > \tr(\Sigma)^{\frac{1}{2} + \eps} + \sqrt{2 \log \frac{1}{\delta}} \right]
    \end{align*} 
    Now,
    \begin{align*}
        &\Pr_{X, v\sim S^{d-1}}\left[ v^T X > \sqrt{(v^T \Sigma v) \cdot 2\log \frac{1}{\delta}} \Big | \|X\| > \tr(\Sigma)^{\frac{1}{2} + \eps} + \sqrt{2 \log \frac{1}{\delta}} \right]\\
        &=1 - \Pr_{X, v \sim S^{d-1}}\left[\|X\| v^T e_1 \le \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta} } \Big | \|X\| > \tr(\Sigma)^{\frac{1}{2}+\eps} + \sqrt{2 \log \frac{1}{\delta}} \right]
    \end{align*}
    We have
    \begin{align*}
        &\Pr_{X, v \sim S^{d-1}}\left[\|X\| v^T e_1 \le \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta} } \Big | \|X\| > \tr(\Sigma)^{\frac{1}{2}+\eps} + \sqrt{2 \log \frac{1}{\delta}} \right]\\
        &\le \Pr_{X, v\sim S^{d-1}} \left[\left(\tr(\Sigma)^{\frac{1}{2} + \eps} + \sqrt{2 \log \frac{1}{\delta}} \right) v^T e_1 \le \sqrt{(v^T \Sigma v) \cdot 2 \log \frac{1}{\delta}} \right]
    \end{align*}
\end{proof}


==> parameter_estimation.tex <==
\section{Estimating a parameter}
We have a distribution family $\{f(\cdot, \theta) | \theta \in \R\}$. Given samples from one such $f(\cdot, \theta)$, we would like to recover $\hat \theta$ close to $\theta$.

\textbf{Solution:} Smoothing. Let $Z_r \sim \mathcal N(0, r^2)$, and let our samples $X \sim f(\cdot, \theta + Z_r)$. $f_r(x, \theta) = \E_{z \sim Z_r} [f(x, \theta + z)]$.

\begin{lemma}
    \begin{align*}
        \frac{f_r(x, \theta + \eps)}{f_r(x, \theta)} = \E_{Z_r | x}\left[e^{\frac{2 \eps Z_r - \eps^2}{2 r^2}} \right]
    \end{align*}
    so that $$s_r(x, \theta) = \E_{Z_r | x} \left[ \frac{Z_r}{r^2}\right]$$
\end{lemma}
\begin{proof}
First, $$p_\theta(z | x) = \frac{p_\theta(z, x)}{p_\theta(x)} = \frac{w_r(z) f(x, \theta + z)}{f_r(x, \theta)}$$

Now,
\begin{align*}
f_r(x, \theta+\eps) &= \int_{-\infty}^\infty w_r(z) f(x, \theta + \eps - z) dz\\
&= \int_{-\infty}^\infty w_r(z+ \eps) f(x, \theta - z) dz\\
&= \int_{-\infty}^\infty p_\theta(z | x) f_r(x, \theta) \frac{w_r(z+\eps)}{w_r(z)}dz\\
&= f_r(x) \E_{Z_r | x} \left[ \frac{w_r(Z_r + \eps)}{w_r(Z_r)}\right]\\
\end{align*}
\end{proof}

It seems like you can sample from $f(x, \theta + Z_r)$ as long as you can write $f(x, \theta + Z_r) = f(x, \theta) + g(Z_r, f(x, \theta))$. Then, you can let your sample $X = \wh X + g(Z_r, \wh X)$ where $\wh X \sim f(x, \theta)$.

For instance, for variance, we can let $X = \wh X + \frac{Z_r}{\theta} \wh X$. Of course, we don't actually have access to $\theta$, but maybe a good initial estimate is enough, or maybe we can choose our $r$ to account for this. Let's assume that our distribution has kurtosis bounded by a constant. So $X = \wh X + \frac{Z_r}{\wh \theta} \wh X$, where $\wh \theta = \theta(1 + O\left(\frac{1}{\sqrt{n}}\right))$. So, $X = \wh X + \frac{Z_r}{\theta}(1 + O(\frac{1}{\sqrt{n}})) \wh X$

So now, we get samples $X \sim f(\cdot, \theta + Z_r\left(1 + O\left(\frac{1}{\sqrt{n}} \right) \right))$. Then, if our initial estimate is within $\theta/\sqrt{n}$, it suffices to set $r$ wrt this width.


==> shifted_covariance_norm_and_trace.tex <==
\begin{corollary}
\label{shifted_covariance_norm}
     Suppose $f_R$ is a $R$-smoothed distribution on $\R^d$ with Fisher information matrix $\I_R$. Let $M \in \R^{d \times d}$ be a symmetric matrix such that $M \succcurlyeq 0$. Then for $\eps \in \R^d$ with $|\eps^T R^{-1} \eps| \le 1/4$, we have,
     \begin{align*}
        \left| \left\|\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] \right\| - \|M \I_R M\|\right| \lesssim \sqrt{\eps^T R^{-1} \eps} \cdot \|M \I_R M\| \cdot \sqrt{\log\left( \sup_{v \in S^{d-1} }\frac{v^T M R^{-1} M v}{v^TM \I_R Mv}\right)}
     \end{align*}
\end{corollary}
\begin{proof}
    Note that for matrix $A \in \R^{d \times d}$,
    $$\|A\| = \sup_{v \in \R^d : \|v\| = 1} v^T A v$$

    So,
    \begin{align*}
        &\left| \left\|\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] \right\| - \|M \I_R M\|\right|\\
        &= \left|\sup_{v: \|v\| = 1} v^T \E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M\right] v - \sup_{v : \|v\| = 1} v^T M \I_R Mv \right|\\
        &\le \sup_{v : \|v\| = 1}\left|v^T \left(\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] - M \I_R M\right)v \right|
    \end{align*}
    Let $v_*$ be the optimizer of the above $\sup$. Then, by the Lemma~\ref{lem:shifted_covariance},
    \begin{align*}
        &\left| \left\|\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] \right\| - \|M \I_R M\|\right| \lesssim \sqrt{\eps^T R^{-1} \eps}(v_*^T M \I_R M v_*) \sqrt{\log \frac{v_*^T M R^{-1} M v_*}{v_*^T M \I_R M v_*}}
    \end{align*}
    Now, for \emph{any} $v \in \R^d$ with $\|v\| = 1$, we have both
    $$v^T M \I_R M v \le \|M \I_R M\|$$
    and
    $$\frac{v^T M R^{-1} M v}{v^T M \I_R M v} \le \sup_{v \in S^{d-1}}\frac{v^T M R^{-1} M v}{v^TM \I_R Mv}$$
    The claim follows.
\end{proof}
\begin{corollary}
\label{cor:shifted_covariance_trace}
    Suppose $f_R$ is a $R$-smoothed distribution on $\R^d$ with Fisher information matrix $\I_R$. Let $M \in \R^{d \times d}$ be a symmetric matrix such that $M \succcurlyeq 0$. Then for $\eps \in \R^d$ with $|\eps^T R^{-1} \eps| \le 1/4$, we have,
    \begin{align*}
        &\left|\tr\left(\E_{x \sim f_R} [M s_R(x+\eps) s_R(x+\eps)^T M]\right) - \tr( M \I_R M)\right|\\
        &\lesssim  \sqrt{\eps^T R^{-1} \eps} \cdot  \tr(M \I_RM) \cdot \sqrt{\log \left(\sup_{v \in S^{d-1}} \frac{v^T M R^{-1} M v}{v^T M\I_RMv}\right)}
    \end{align*}
\end{corollary}

\begin{proof}
    Note that for matrix $A \in \R^{d \times d}$,
    $$\tr(A) = \sum_{i=1}^d e_i^T A e_i$$
    So, by the Lemma~\ref{lem:shifted_covariance},
    \begin{align*}
        &\left|\tr\left(\E_{x \sim f_R} [M s_R(x+\eps) s_R(x+\eps)^T M]\right) - \tr(M \I_R M)\right|\\
        &= \left|\sum_{i=1}^d e_i^T \left(\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] - M \I_R M \right)e_i\right|\\
        &\le \sum_{i=1}^d\left| e_i^T \left(\E_{x \sim f_R}\left[M s_R(x+\eps) s_R(x+\eps)^T M \right] - M \I_R M \right)e_i\right|\\
        &\lesssim \sum_{i=1}^d \sqrt{\eps^T R^{-1} \eps} (e_i^{T} M \I_R M e_i) \sqrt{ \log \frac{e_i^T M R^{-1} M e_i}{e_i^T M \I_R M e_i}} 
    \end{align*}
    Now, for any vector $v \in \R^d$,
    $$\frac{v^T M R^{-1} M v}{v^T M \I_R M v} \le \sup_{v \in S^{d-1}} \frac{v^\top M R^{-1} M v}{v^\top M\I_RM v}$$
    So,
    \begin{align*}
        &\left|\tr\left(\E_{x \sim f_R} [M s_R(x+\eps) s_R(x+\eps)^T M]\right) - \tr(M \I_R M)\right|\\
        &\lesssim \sum_{i=1}^d \sqrt{\eps^T R^{-1} \eps} (e_i^T M \I_R M e_i) \sqrt{ \log \left(\sup_{v \in S^{d-1}} \frac{v^\top M R^{-1} M v}{v^\top M\I_RM v}\right)}\\
        &= \sqrt{\eps^T R^{-1} \eps} \cdot  \tr(M\I_R M) \cdot \sqrt{\log \left(\sup_{v \in S^{d-1}} \frac{v^\top M R^{-1} M v}{v^\top M\I_RM v}\right)}
    \end{align*}
\end{proof}


==> subgaussian_marginals.tex <==
\begin{theorem}[Subgaussian marginals]
  Let $x$ be a mean zero random vector in $\R^d$ that is
  $\Sigma$-subgaussian, i.e., it satisfies
  \[
    \E[e^{\lambda \inner{x, v}}] \leq e^{\lambda^2 v^T \Sigma v}
  \]
  for every vector $v$.  Then for any $\gamma > 0$,
  \[
    \Pr[\norm{x} \geq (1+\gamma)\sqrt{\Tr(\Sigma)}] \leq e^{-\frac{\gamma^2}{4} \frac{\Tr(\Sigma)}{\norm{\Sigma}}}.
  \]

\end{theorem}


This seems to match the Gaussian concentration bound in
(\url{https://arxiv.org/pdf/1906.04280.pdf}), of
$\sqrt{\Tr(\Sigma)} + \sqrt{2 \norm{\Sigma} \log \frac{1}{\delta}}$,
to within a $\sqrt{2}$ factor in the second term.  (It's also
\emph{not} tight for the analysis, it's sloppy with that constant.)
The Hanson-Wright inequality also matches this but loses constants and
requires the coordinates of $x$ to be independent.

\begin{proof}
  Define
  \[
    \alpha := \Pr[\norm{x} \geq (1+\gamma)\sqrt{\Tr(\Sigma)}].
  \]
  so by Markov's inequality applied to $e^{\lambda^2 \norm{x}^2}$,
  \[
    \alpha \leq \frac{\E[e^{\lambda^2 \norm{x}^2}]}{e^{\lambda^2 (1+\gamma)^2 \Tr(\Sigma)}}
  \]
  for any $\lambda$.
  
  Draw $v \sim N(0, I)$ independently of $x$, and consider the
  MGF of $\inner{x, v}$.

  On the one hand, for fixed $x$ as a distribution over $v$,
  $\inner{x, v} \sim N(0, \norm{x}^2)$.  Thus
  \[
    \E_x[ \E_v[e^{\lambda \inner{x, v}}]] = \E_x[e^{\lambda^2 \norm{x}^2}]
  \]
  Therefore we have
  \begin{align}\label{eq:mgflower}
    \alpha \leq \E_{x,v}[e^{\lambda \inner{x, v}}] \cdot e^{- \lambda^2 (1 + \gamma)^2\Tr(\Sigma)}.
  \end{align}
  for any $\lambda$.

  On the other hand, for fixed $v$ as a distribution over $x$, the
  $\Sigma$-subgaussian assumption implies
  \[
    \E_x[e^{\lambda \inner{x, v}}] \leq e^{\lambda^2 v^T \Sigma v}.
  \]
  Let the eigenvalues of $\Sigma$ be
  $\sigma_1^2 \geq \sigma_2^2 \geq \dotsb \geq \sigma_d^2$.  Then
  $v^T \Sigma v$ is a generalized chi-squared distribution,
  distributed as $\sum_i w_i^2$ for independent Gaussian variables
  $w_i \sim N(0, \sigma_i^2)$.  It is well known (see XXX) that
  $w^2$ for $w \sim N(0, 1)$ is $(2, 4)$-subgamma, i.e.,
  \[
    \E[e^{\lambda (w^2-\E[w^2])}] \leq e^{2 \lambda^2} \qquad \forall \abs{\lambda} \leq \frac{1}{4}.
  \]
  (easy to check,
  $\E[e^{\lambda w^2}] = \frac{1}{\sqrt{1-2\lambda}}$).  Therefore
  $\sum w_i^2$ is $(2 \sum_i \sigma_i^4, 4 \max \sigma_i^2)$ =
  $(2 \norm{\Sigma}_F^2, 4 \norm{\Sigma})$-subgamma.  Since
  $\norm{\Sigma}_F^2 \leq \norm{\Sigma}\Tr(\Sigma)$, $v^T \Sigma v$ is
  also $(2 \norm{\Sigma}\Tr(\Sigma), 4 \norm{\Sigma})$-subgamma.

  Including the mean term as well ($\E[v^T \Sigma v] = \Tr(\Sigma)$), we have
  \[
    \E_v[e^{\lambda^2 v^T \Sigma v}]\leq e^{\lambda^2 \Tr(\Sigma)} \cdot e^{2 \lambda^4 \Tr(\Sigma) \norm{\Sigma}} \qquad\forall \lambda^2 \leq \frac{1}{4\norm{\Sigma}},
  \]
  and so
  \begin{align}\label{eq:mgfupper}
    \E_{x,v}[e^{\lambda \inner{x, v}}] \leq \E_v[e^{\lambda^2 v^T \Sigma v}]  \leq e^{\lambda^2 \Tr(\Sigma)(1 + 2\lambda^2 \norm{\Sigma})} \qquad\forall \lambda^2 \leq \frac{1}{4\norm{\Sigma}}.
  \end{align}
  Combining with~\eqref{eq:mgflower},
  \[
    \alpha \leq e^{\lambda^2 \Tr(\Sigma)(2\lambda^2 \norm{\Sigma} - 2 \gamma - \gamma^2)} \qquad\forall \lambda^2 \leq \frac{1}{4\norm{\Sigma}}.
  \]
  or
  \[
    \alpha \leq e^{- \gamma(1+\gamma) \lambda^2 \Tr(\Sigma)} \qquad \forall \lambda^2 \leq \min(\frac{1}{4\norm{\Sigma}}, \frac{\gamma}{2\norm{\Sigma}}).
  \]
  Setting $\lambda$ to the max of this range, we have
  \[
    \alpha \leq e^{- \frac{\Tr(\Sigma)}{\norm{\Sigma}} \min(\frac{\gamma+\gamma^2}{4}, \frac{\gamma^2 + \gamma^3}{2})} \leq e^{- \frac{\gamma^2}{4}\frac{\Tr(\Sigma)}{\norm{\Sigma}}}
  \]
  as desired.
\end{proof}

\begin{remark}
  To extend to subgamma variables, it's slightly annoying since the
  exponential scale of $\inner{x, v}$ has to scale with $\norm{v}$.

  Of course, with overwhelming probability we will have
  $\norm{v} = \Theta(\sqrt{d})$ in our setting, so probably we can
  restrict to that somehow.  And ultimately care that we can set
  $\lambda = \sqrt{\frac{\gamma}{2 \norm{\Sigma}}}$.  So most likely
  it works as long as:
  \[
    \E[e^{\lambda \inner{x, v}}] \leq e^{\lambda^2 v^T \Sigma v}
  \]
  for all $\norm{v} = \sqrt{d}$ and
  $\abs{\lambda} \leq \sqrt{\frac{\gamma}{2 \norm{\Sigma}}}$, i.e.,
  that $\inner{x, v}$ is
  $(v^T \Sigma v, \sqrt{\frac{2 \norm{\Sigma}}{\gamma}})$-subgamma.
\end{remark}

